Incorporating Word Sense Disambiguation in Neural Language Models

We present two supervised (pre-)training methods to incorporate gloss definitions from lexical resources into neural language models (LMs). The training improves our models' performance for Word Sense Disambiguation (WSD) but also benefits general language understanding tasks while adding almost no parameters. We evaluate our techniques with seven different neural LMs and find that XLNet is more suitable for WSD than BERT. Our best-performing methods exceeds state-of-the-art WSD techniques on the SemCor 3.0 dataset by 0.5% F1 and increase BERT's performance on the GLUE benchmark by 1.1% on average.

==> tables/base_large_table.tex <==
\begin{table}[H]
\centering
 \resizebox{.35\textwidth}{!}{ 
    \begin{tabular}{l ccc} \toprule
    \textbf{System} & \textbf{SE2} & \textbf{SE13} & \textbf{All} \\ \midrule
    BERT$_{BASE}$ \citeyear{DevlinCLT19} & 77.78 & 76.52 & 76.59 \\
    BERT$_{LARGE}$ \citeyear{DevlinCLT19} & 78.26 & 76.46 & 76.67 \\
    \bottomrule
    \end{tabular}
    }
\caption{Model size comparison largest evaluation sets.}
\label{table:base_large}
\end{table}

% \begin{table}[H]
% \centering
%  \resizebox{.48\textwidth}{!}{ %TR: this is the commando I mentioned to you. I also changed the hlines to top/mid/bottom rule
%     \npdecimalsign{.}
%     \nprounddigits{2}
%     \begin{tabular}{l n{5}{2} n{5}{2} n{5}{2}} \toprule
%     \textbf{System} & \textbf{Senseval2} & \textbf{SemEval2013} & \textbf{All} \\ \midrule
%     BERT$_{BASE}$ \citeyear{DevlinCLT19} & 77.78264680105171 & 76.52068126520681 & 76.5889976561423 \\
%     BERT$_{LARGE}$ \citeyear{DevlinCLT19} & 78.2646801051709 & 76.45985401459855 & 76.67172204604991 \\
%     \bottomrule
%     \end{tabular}
%     }
% \caption{Evaluation of the two different model sizes of BERT with the two largest evaluation sets of \cite{RaganatoCN17}.}
% \label{table:base_large}
% \end{table}

==> tables/dataset_glue_table.tex <==
\begin{table*}[htb]
\centering
 \resizebox{0.94\textwidth}{!}{
    \begin{tabular}{llcccccccc} \toprule
     & & MNLI & QQP & QNLI & SST-2 & CoLA & STS-B & MRPC & RTE \\
     & & 392k & 363k & 108k & 67k & 8.5k & 5.7k & 3.5k & 2.5k \\ \midrule
    \multirow{3}{*}{Train} & Words & 11\,695k & 8\,050k & 3\,818k & 633k & 65k & 114k & 160k & 130k \\
    {} & Polysemous & 5\,205k & 3\,452k & 1\,439 & 366k & 23k & 51k & 65k & 50k \\
    {} & Relation (\%) & 44,5& 42,9 & 37,7 & 57,8 & 35,5 & 44,9 & 40,9 & 39,0 \\ \midrule
    \multirow{3}{*}{Test} & Words & 286k & 893k & 205k & 17k & 8k & 34k & 17k & 14k \\
    {} & Polysemous & 126k	& 382k & 78k & 9k & 2k & 15k & 7k & 5k \\
    {} & Relation (\%) & 44.2 & 42.8 & 8.2 & 54.1 & 34.7 & 46.4 & 41.9 & 38.7 \\
    \bottomrule
    \end{tabular}
    }
\caption{The number of polysemous words in relation to the number of total words in the GLUE evaluation datasets except for WNLI. Under each dataset is the number of training examples.}
\label{table:glue_polysemy}
\end{table*}

==> z_take_out.tex <==
\begin{abstract}
Word sense disambiguation (WSD) is the task of finding the most suitable sense of an ambiguous word in a particular context.
Recent publications have shown the effectiveness of incorporating lexical resources in neural language models for WSD.
These methods perform well on the disambiguation task but lack transfer learning capabilities on typical downstream applications.
We present \methodName~(\textbf{G}loss \textbf{i}ncorporating \textbf{l}inguistic \textbf{B}idirectional \textbf{E}ncoder \textbf{R}epresentations from \textbf{T}ransformers), a set of supervised (pre-)training methods for incorporating gloss definitions from lexical resources to leverage WSD capabilities in neural language models. \methodName's training focusses on WSD and keeps its capabilities during transfer learning to other tasks while adding almost no additional parameters. We evaluate our technique on 15 different downstream tasks, e.g., sentence pair classification, WSD, and show our approaches achieve up to 4.5\% increase in F1-score over state-of-the-art methods on SemEval2007 (3.1\% on average on SemEval and Senseval datasets), and increase performance by 2.9\% on the GLUE benchmark over BERT.
\end{abstract}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% INTRODUCTION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Pre-trained word representations have become crucial for neural language models \cite{MikolovCCD13,DaiL15,PetersNIG18,RadfordWCL18,HowardR18}. Despite their robustness in many tasks, word representations often fall short in intrinsic linguistic properties, such as the representation of multiple word senses (polysemy). For example, phrases containing the word {\itshape java} are ambiguous as {\itshape java} can refer to the programming language, an island, or a coffee.
Word Sense Disambiguation (WSD) tries to determine the meaning of words given a context and is arguably one of the oldest challenges in natural language processing (NLP)~\cite{Weaver1955,NavigliP12}. In knowledge-based methods \cite{CamachoColladosPN15}, lexical databases (e.g., WordNet~\cite{Miller95a,Fellbaum98a}, ConceptNet \cite{LiuS04}, BabelNet~\cite{NavigliP12}) are used as a taxonomy to help categorize the relationship between words and their meaning. While unsupervised techniques~\cite{ChaplotS18} do not rely on annotated data to perform disambiguation, supervised-based ones~\cite{PasiniN20} require sufficient data to learn the multiple meanings of a word. 

Recent language models such as BERT~\cite{DevlinCLT19} and ELMo~\cite{PetersNIG18} try to overcome linguistic issues replacing unique word representations with context-dependent embeddings. However, current state-of-the-art neural language models fail to represent intrinsic linguistic properties, as they often ignore valuable information (e.g., lemma, gloss\footnote{Brief definition of a cognitive synonym set (synset)~\cite{Miller95a}.}) of word senses present in lexical databases. Furthermore, as our experiments support, there should be a positive correlation between the language models' ability to disambiguate word senses and overall performance on NLP tasks.

Previous work uses different architectures to perform WSD. \newcite{KagebackS16} train a bidirectional long short-term memory network (Bi-LSTM\footnote{Referenced as BLSTM by the authors.}) using context sentences as input to obtain word senses with shared weights between word types.
Gloss-augmented WSD neural networks (GAS)~\cite{LouLHX2018b} model the semantic relationship between context words and WordNet glosses in a memory network~\cite{SukhbaatarSWF15}.
Co-attention neural networks (CAN) and its hierarchical model (HCAN)~\cite{LuoLHX18} use a co-attention mechanism to map the context of polysemous words to semantically similar gloss words.

The most recent works in the disambiguation domain modify neural language models, e.g., BERT, to perform WSD.
GlossBERT (Sent-CLS-WS)~\cite{HuangSQH19} transforms the WSD tasks into a weakly supervised binary classification of an annotated sentence and a gloss from WordNet using BERT.
KnowBert-W+W~\cite{PetersNLS19} uses a word-to-entity attention mechanism to embed the lexical resources of WordNet and Wikipedia into BERT.
\newcite{DuQS19} transform token embeddings and glosses into a classification unit to predict the correct sense of tokens. SenseBERT~\cite{LevineLDP19} weakly supervises the masked language model (MLM) objective from BERT to predict WordNet's super sense simultaneously to the masked word. We provide a more in-depth view on the related literature of WSD and neural language models in Section \ref{sec:rw}.

We argue that current state-of-the-art focuses primarily on the WSD domain without using the potential of WSD for other NLP tasks. We also suggest modifying the prediction step from sequential binary classification to parallel multi-classification constructs a more natural prediction head as previous literature showed \cite{KagebackS16}.

In this work, we improve BERT's ability to perform WSD and its capabilities in other NLP downstream tasks through an inductive transfer learning manner.
We propose GilBERT, a set of general supervised methods to perform WSD using neural language models. Our pre-training method incorporates knowledge from WordNet in BERT. Additionally, we frame WSD as a multi-classification of candidate glosses with state-of-the-art performance. We make all source code and datasets publicly available\footnote{\url{https://anonymous.4open.science/r/c4d5f346-dd85-410e-b362-d0ff402a49c7/}}.

Our best performing method in WSD improves the F1-score in 3.1\% over state-of-the-art on five standardized test sets proposed by \newcite{RaganatoCN17}. \methodName~pre-training methods also increase performance by 2.9\% on GLUE benchmark~\cite{WangSMH19} when compared to recent work \cite{HuangSQH19} and the official BERT weights \cite{DevlinCLT19}. Our methodology is presented in details in Section~\ref{sec:methods} and the experimental results are discussed in Section~\ref{sec:experiments}. 

These models are trained on large unlabeled corpora and most of times neglect the valuable information of word senses present in LKB (e.g., gloss\footnote{Brief definition of a cognitive synonym set (synset)~\cite{Miller95a}.}). As our experiments support, there should be a positive correlation between the LM's ability to disambiguate words and overall performance in other NLP tasks. We argue the current research in \wsd does not explore transferring the acquired knowledge to other tasks (e.g., text-classification).


We propose \methodName, a set of general supervised methods to perform \wsd using neural \LM.
Our technique incorporates knowledge from WordNet in the pre-training phase, improving \LM~s performance in language understanding \footnote{\url{https://anonymous.4open.science/r/c4d5f346-dd85-410e-b362-d0ff402a49c7/}}.

%TR: ORIG: The presented pre-training methods achieve state-of-the-art performance in WSD and increases generalization on other NLP tasks~\cite{WangSMH19} when compared to recent work \cite{HuangSQH19} and the official BERT weights \cite{DevlinCLT19}. Our methodology is presented in details in Section~\ref{sec:methods} and the experimental results are discussed in Section~\ref{sec:experiments}.

% Closing statement - work towards methods

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% RELATED WORK
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}
\label{sec:rw}

Knowledge-based WSD methods use lexical resources such as WordNet~\cite{Miller95a,Fellbaum98a} and exploit different types of knowledge, e.g., graph structure, and glosses. Glosses are crafted definitions of word sense meanings and were first used in the Lesk algorithm~\cite{Lesk86a} and its variations~\cite{basile2014enhanced,BanerjeeP02a}.

% Neural approaches
More recently, neural network-based models~\cite{BengioDVJ03,MikolovSCC13,BojanowskiGJM17} have gained much attention in the NLP community, mainly because of their success to capture latent semantic content and excellent results in NLP tasks, such as word similarity~\cite{NeelakantanSPM14}, text classification \cite{RuasFGd20}, and topic categorization~\cite{PilehvarCNC17}. \newcite{RuasGA19} use a gloss vector representation, from WordNet~\cite{Fellbaum98a}, and a pre-trained word2vec~\cite{MikolovSCC13} model to disambiguate polysemous words in a fixed context window. Likewise, we also consider the glosses in WordNet, but we rely on the neural network do identify the correct sense of a word given its context.

% Bring transformers 
%BERT Direction - tasks and following publications
Based on the Transfomer~\cite{VaswaniSPU17} architecture, BERT~\cite{DevlinCLT19} proposes two pre-training tasks to capture general aspects of the language, i.e., \textit{Masked Language Model} (MLM) and \textit{Next Sentence Prediction} (NSP). MLM uses deep bidirectional architecture to build a language model, masking out random tokens in the input. The NSP task identifies if two sentences are semantically connected. Different from ELMo~\cite{PetersNIG18} and GPT~\cite{RadfordWCL18}, BERT considers left-to-right and right-to-left context simultaneously, allowing a more realistic representation of the language. Even though ELMo does use two Bi-LSTM, their weights are not shared during training. On top of MLM and NSP, BERT requires fine-tuning to specific tasks to adjust its weights accordingly. 

The same way word2vec~\cite{MikolovSCC13} inspired many models in NLP~\cite{LeM14,IacobacciPN15,PilehvarC16,BojanowskiGJM17,RuasGA19,RuasFGd20}, BERT success echoed in the literature with recent models as well ~\cite{LanCGG19,LiuOGD19,SanhDCW19,BeltagyLC19a,HuangSQH19,YangDYC19,ClarkLLM20}. We move towards improving BERT representation and generalization over different tasks with WordNet's ~\cite{Fellbaum98a} lexical structure.

ALBERT~\cite{LanCGG19}, DistilBERT~\cite{SanhDCW19}, and RoBERTa~\cite{LiuOGD19} either boost BERT's performance through hyperparameter adjustments or make it less computationally expensive. SciBERT~\cite{BeltagyLC19a} and DocBERT~\cite{AdhikariRTL19} adjust their predecessor's fine-tuning tasks for the scientific domain and document classification, respectively. ELECTRA~\cite{ClarkLLM20} changes the MLM task to corrupt words in a sentence instead of just masking them. The replaced tokens are substituted with artificially generated ones from a small masked language model in a noise contrastive learning process~\cite{GutmannH10}. In XLNet~\cite{YangDYC19}, a permutation language modeling predicts one word given its preceding context in a random manner. 

Gloss-augmented WSD neural networks (GAS)~\cite{LouLHX2018b} model the semantic relationship between context words and WordNet glosses in a memory network~\cite{SukhbaatarSWF15}.Co-attention neural networks (CAN) and its hierarchical model (HCAN)~\cite{LuoLHX18} use a co-attention mechanism to map the context of polysemous words to similar gloss words.

Directly related to our work, GlossBERT~\cite{HuangSQH19} uses WordNet's glosses to fine-tune BERT in the WSD task. They modify the NSP task to classify a marked word $w_{i}$ in a sentence $A$ into one of the possible gloss definitions in sentence $B$, also containing $w_{i}$. We believe highlighting $w_{i}$ with additional tokens introduces a bias to the network. Even though GlossBERT achieves excellent results in the WSD task, it loses in generalization when applied to other NLP tasks, as we showed in Section~\ref{sec:experiments}. Our model incorporates WordNet's knowledge more organically, using the positional encoding to link $w_{i}$ and prospective gloss definition without requiring additional token insertion. \newcite{DuQS19} fine-tune BERT in the WSD task using word-sense definitions from WordNet combining an encoder and classifier. Their encoder extracts polysemes' features from sentences, and the classifier uses them to predict the senses. SenseBERT~\cite{LevineLDP19} also incorporates WordNet and modifies the MLM to predict supersenses of the masked words. The word-sense information improves BERT's self-supervision incorporating semantic relations from WordNet.

KnowBERT~\cite{PetersNLS19} incorporates knowledge bases (KB) into BERT (e.g., WordNet, Wikipedia) with a Knowledge Attention and Recontextualization mechanism. Their technique uses mention-spans to retrieve entity embeddings from a KB, update the mention-span embeddings with the linked information, and recontextualize the entity embeddings with altered multi-head attention. Their multi-head self-attention is modified so that a word-piece can attend to all entity embeddings in the context. \newcite{PetersNLS19} best-performing model, i.e., KnowBERT combining Wikipedia and WordNet (KnowBERT-W+W), achieves better results than both BERT models (base and large). However, KnowBERT-W+W adds over 400 million parameters when compared to BERT$_{base}$ and is 32\% slower. The overhead in computation time and the number of parameters can be a limiting factor. \methodName~does not require recurrent embeddings adjustments from the KB or use word-piece attention, resulting in a less expensive alternative. Other feature-based approaches for semantic relationships (e.g., hypernymy), even though not directly related to our contributions, are also discussed in the literature~\cite{VialLS19}.

\cite{BlevinsZ20} propose BEM, a model to encode a target word with its surrounding context and the gloss of each sense in separate encoders. Their two encoders are learned simultaneously from the \wsd objective. EWISER~\cite{BevilacquaN20}, an extension of \cite{KumarJST19} uses different word embeddings as input to include semantic relations (e.g., hypernym) in their structure. LMMS~\newcite{LoureiroJ19} combines $k-$NN using the most frequent sense (MFS) in WordNet with BERT embeddings. GLU~\cite{HadiwinotoNG19} integrates contextualized word representations in \wsd. Even though the previous techniques enhance their semantic representations via context, external knowledge, or MFS, they do not explore how their techniques generalize to other NLP tasks. Yet, \methodName, often outperforms preceding techniques in WSD and obtains the highest score in 7 out of 9 GLUE tasks.

\cite{BlevinsZ20} propose BEM, a model to encode a target word with its surrounding context and the gloss of each sense in separate encoders. Their two encoders are learned simultaneously from the \wsd objective. EWISER~\cite{BevilacquaN20}, an extension of \cite{KumarJST19} uses different word embeddings as input to include semantic relations (e.g., hypernym) in their structure. LMMS~\newcite{LoureiroJ19} combines $k-$NN using the most frequent sense (MFS) in WordNet with BERT embeddings. GLU~\cite{HadiwinotoNG19} integrates contextualized word representations in \wsd. Even though the previous techniques enhance their semantic representations via context, external knowledge, or MFS, they do not explore how their techniques generalize to other NLP tasks. Yet, \methodName, often outperforms preceding techniques in WSD and obtains the highest score in 7 out of 9 GLUE tasks.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%TABLE SEMEVAL%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[htb]
\centering
 \resizebox{1\textwidth}{!}{ %TR: this is the commando I mentioned to you. I also changed the hlines to top/mid/bottom rule
    \begin{tabular}{lcccccc} \toprule
    \textbf{System} & \textbf{SemEval2007} & \textbf{Senseval2} & \textbf{Senseval3} & \textbf{SemEval2013} & \textbf{SemEval2015} & \textbf{All} \\ \midrule
    MFS (Most Frequent Sense)                & 54.5 & 65.6 & 66.0 & 63.8 & 67.1 & 64.8 \\
    Bi-LSTM                                  & - &	71.1 &	68.4 &	64.8 &	68.3 & 68.4 \\
    Bi-LSTM+att.+LEX+pos                     & 64.8 & 72.0 & 69.1 & 66.9 & 71.5 & 69.9  \\\hdashline
    GAS ext (Linear)                         & - & 72.4 & 70.1 & 67.1 & 72.1 & 70.4 \\
    GAS ext (Conc.)                  &  - & 72.2 & 70.5 & 67.2 & 72.6 & 70.6 \\
    CAN                                      &  - & 72.2 & 70.2 & 69.1 & 72.2 & 70.9 \\
    HCAN                                     & - & 72.8 & 70.3 & 68.5 & 72.8 & 71.1\\
    BEM                                      & 74.5 & 79.4 & 77.4 & 79.5 & 81.7 & 79.0 \\
    EWISER$_{hyper}$                           & 71.0 & 80.8 & 79.0 & 80.7 & 81.8 & 78.6 \\
    LMMS$_BERT$                              & 68.1 & 76.3 & 75.6 & 75.1 & 77.0 & 75.4 \\
    GLU (1sent+1sur)\cite{HuangSQH19}        & 68.1 & 75.5 & 73.6 & 71.1 & 76.2 & 74.1 \\    
    GlossBERT(\citeyear{HuangSQH19})        & 72.5 & 77.7 & 75.2 & 76.1 & \textbf{80.4} & 77.0 \\ 
    BERT for WSD                             & - & 76.4 & 74.9 & 76.3 & 78.3 & 76.3 \\
    KnowBERT-W+W                             & - & - & - & - & - & 75.1 \\\hdashline
    \methodName~BGP         & 70.4 & 77.8 & 74.9 & 76.4 & 78.8 & 76.4  \\
    \methodName~BGP-M     & 72.9 & 78.2 & 75.5 & 76.3 & 79.5 & 77.0 \\
    \methodName~MCGP (k=8) & \textbf{76.7} & \textbf{80.8} & \textbf{80.7} & \textbf{79.9} & 79.3 & \textbf{80.1} \\ \bottomrule
    \end{tabular}
    }
\caption{Test results, scored by the fine-grained English all-words WSD evaluation framework \cite{RaganatoCN17}. All methods report F1 calculated by the official scoring scripts provided by~\newcite{RaganatoCN17}. \textbf{Bold} font indicates the best result per dataset.}
\label{table:semeval}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% METHODS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent \textbf{Binary Gloss Prediction (BGP)} is our baseline method to perform WSD in pre-trained language models. BGP addresses the problem of imbalanced examples by using the focal loss function~\cite{LinGGH17}, a state-of-the-art method to tackle class imbalance in object detection from camera images. Although accumulated negative examples do not dominate the loss in our experiments, they are certainly affected. Adopting the focal loss function allows us to improve the model's convergence, resulting in higher performance. Additionally, we include a weak supervision signal using segment embeddings in the training procedure to reduce the model bias towards text in comparison to token insertion (Section~\ref{sec:sgb}). 

\noindent \textbf{BGP with Masked Language Modeling (BGP-M)} builds on top of the BGP model and incorporates a MLM objective. The additional objective aims to maintain language model features while optimizing the model for disambiguation. MLM improves our model task-specific performance and generalization capabilities on a variety of NLP downstream tasks (Section~\ref{sec:sgb-m}).

\noindent \textbf{Multiple-Choice Gloss Prediction (MCGP)} incorporates additional context candidate glosses and simplifies the prediction step, treating WSD as a multiple-choice problem. MCGP increases the baseline performance in WSD and addresses the class imbalance implicitly (Section~\ref{sec:sgmc}).

%%%%%%%%%%%
% BGP
%%%%%%%%%%%
In the BGP task we pair (i) a sentence containing a polysemous target word with (ii) a prospective gloss definition from a lexical database (e.g., WordNet) for this word. Let $W = (w_1, \dots, w_n)$ be a word sequence of a sentence, where $w_i$ is a polysemous word. WordNet provides $S_i = \{s_1, \dots, s_m\}$ possible senses for word $w_i$ with corresponding glosses $G_i = \{g_1, \dots, g_m\}$, which are also individual sentences.

We build an annotated corpus using WordNet glosses to perform the BGP.
For a sentence $W$, each polysemous word $w_i$ points to correct WordNet senses $\widetilde{S}_i \subset S_i$. We retrieve the glosses' candidates $G_i$ to create $|G_i|$ pairs of the sentence $W$ and glosses $g_j$, with $g_j \in G_i$. If $g_j$ corresponds to the desired meaning of our polysemous target word $w_i$ (which is the case if $s_j \in \widetilde{S}_i$), we classify the pair as a positive example ($y=1$), otherwise as negative ($y=0$).
As the number of correct senses for a polysemous word is much smaller than the total number of senses for a word, labels are often imbalanced. We support evidence on the label imbalance and resulting underfitting for several WSD benchmarks in Section~\ref{sec:datasets}.

For notation convenience, we assume the token level position is identical to the word level position (e.g., no word has been split into multiple sub-words). We add the same segment embedding $A$ to all tokens in the sentence, except for the ambiguous tokens, e.g., $\{w_1,...,w_n\} \setminus w_i$. The gloss' tokens and ambiguous ones $\{g_{m1},...,g_{mk}\} \cup \{w_i\}$ are added to another segment embedding $B$ before processing in BERT.

To perform classification, \newcite{DuQS19} used the token embedding of a polysemous word. However, \newcite{HuangSQH19} showed, that classification on top of the aggregate representation improves the results in WSD.
Therefore, we obtain the final hidden representation of the ``[CLS]" token, namely $C \in \mathbb{R}^H$; where $H$ is the embedding size. 
We apply a weight matrix $W_{{\scaleto{BGP}{4pt}}} \in \mathbb{R}^{H \times 2}$ transforming $C$ (together with a bias $B_{{\scaleto{BGP}{4pt}}} \in \mathbb{R}^{2}$) into a binary space and calculate the probability to whether the gloss is appropriate for the ambiguity in context as Eq.~\ref{eq:binary_probs} shows.

\begin{equation}
    \label{eq:binary_probs}
    p = \textrm{softmax}(C~W_{\scaleto{BGP}{4pt}}^T + B_{\scaleto{BGP}{4pt}})
\end{equation}

To optimize the model for learning whether a gloss is correct for the annotated ambiguous word, ~\newcite{HuangSQH19} and~\newcite{DuQS19} used the standard cross-entropy loss function (Eq.~\ref{eq:cross_entropy}).

\begin{align}
    \label{eq:cross_entropy}
    \textrm{CE}(p,y) = \begin{cases}
        - \log(p)& \textrm{if y = 1}\\
        1 - \log(1-p)& \textrm{otherwise}
    \end{cases}
\end{align}

Unfortunately, the class imbalance and rare occurrence of challenging examples encountered during training hinder the cross-entropy loss. Easily classified negatives comprise parts of the loss, which obstructs the gradient direction. Thus, we propose to apply a weighted loss function, a popular approach to mitigate the class imbalance in object detection from camera images~\cite{RenHGS15,RedmonF18}. The focal loss~\cite{LinGGH17} (Eq.~\ref{eq:focal_loss}) reshapes the cross-entropy loss function, giving less weight to easy examples and forces the training to focus on challenging polysemous words.

\begin{equation}
    \label{eq:focal_loss}
    \text{FL}(p, y) = \begin{cases}
    
    -(1-p)^{\gamma} \log(p)& \textrm{if y = 1}\\
    -(1+p)^{\gamma} \log(1 - p)& \textrm{otherwise}
    \end{cases}
\end{equation}

Following~\newcite{HuangSQH19}, we insert the target word $w_{i}$ before the gloss as one weak supervision signal. Furthermore, for all methods, we map the word level label positions to token level positions. We use segment embeddings to map polysemous words to gloss words and to distinguish this mapping from the context words. Hence, creating another weak supervision signal with segment embeddings. As the WordPiece tokenizer may split words into multiple sub-words, a token-level transformation is required.

Pre-trained models serve as a valuable feature extractor that can be optimized to new task-specific objectives in a straight forward manner~\cite{DevlinCLT19,RadfordWCL18}. However, optimizing a specific task might disregard previously learned language model capabilities. The WSD task is special, as we can assume when a language model is capable of disambiguation, its ability to perform well on other tasks may increase. For this reason, we want to keep language modeling features while learning WSD. Transfer learning between language modeling and WSD increases the likelihood of understanding polysemous words in other co-related tasks, improving the overall performance. 
In Appendix~\hyperref[appx:A]{A}, we discuss the correlation between WSD and other NLP tasks concerning the number of polysemous words.

For BGP, the task-specific objective is to predict whether the appended gloss explains the correct meaning of a word in a sentence. The corresponding objective function is the focal loss function between the network's prediction and the ground truth label as Eq.~\ref{eq:focal_loss} shows.

%%%%%%%%%
%  BGP-M
%%%%%%%%%

In BGP-M, we perform two forward passes through BERT with similar sentence-gloss pairs. The first pass uses the original pair of a context sentence and gloss. Next, it applies a weight matrix to the final hidden vector token embedding resulting in a binary classification for WSD (Eq.~\ref{eq:binary_probs}). In the second pass, we replace words in the sentence and gloss with a ``[MASK]" token, a random token, or the same token with equal probabilities from~\newcite{DevlinCLT19}.
The BGP-M procedure is exemplified in Figure~\ref{fig:BGP-M}.

In the last layer of the neural language model we obtain each mask token embedding $M_j \in \mathbb{R}^H$ and apply a weight matrix $W_{{\scaleto{BGP-M}{4pt}}} \in \mathbb{R}^{V \times H}$ together with a bias $B_{{\scaleto{BGP-M}{4pt}}} \in \mathbb{R}^V$. This operation results in a probability vector of vocabulary size $V$, as Eq.~\ref{eq:mask_output} shows.

\begin{equation}
    \label{eq:mask_output}
    \widetilde{p}_j = \text{softmax}(M_j W_{{\scaleto{BGP-M}{4pt}}}^T + B_{{\scaleto{BGP-M}{4pt}}})
\end{equation}

We sum the two objectives, i.e. the task-specific WSD focal loss and the MLM cross entropy loss, to obtain the final loss function $\mathcal{L}_1$ described in Eq.~\ref{eq:focal_mlm_loss}, where $l$ is the number of masked words, $\widetilde{y}_j \in \{0, 1\}^V$ is the one-hot encoding for a masked word $w_j$, and $\widetilde{p}_j \in \mathbb{R}^V$ is the probability vector for $w_j$.

\begin{equation}
    \label{eq:focal_mlm_loss}
    \mathcal{L}_1(p, y) = \text{FL}(p,y) + \sum_{k=1}^l \text{CE}(\widetilde{p}_k,\widetilde{y}_k)
\end{equation}

%%%%%%%%
% MCGP
%%%%%%%%

\subsection{Multiple-Choice Gloss Prediction (MCGP)}
\label{sec:sgmc}
Like~\newcite{KagebackS16}, we assume a parameterized softmax classification of candidate glosses can improve our model's performance. Therefore, we propose to treat WSD as a multiple-choice problem. In MCGP, we create $k$ pairs composed of a context sentence, including a polysemous word, and a possible gloss. The general procedure is exemplified for $k=3$ in Figure \ref{fig:MCGP}.

The corresponding ground truth label is a one-hot encoding vector $y \in \{0, 1\}^{k}$.
To obtain representations for each sentence gloss pair, we forward $k$ pairs through the neural network in parallel and obtain each embedding of the ``[CLS]” token $C \in \mathbb{R}^H$. A weight matrix $U \in \mathbb{R}^H$ transforms the embedding space intto a single dimension, which, together with a bias $B \in \mathbb{R}$, forms the intermediate output as Eq.~\ref{eq:multiple_choice_outputs} shows.

\begin{equation}
    \label{eq:multiple_choice_outputs}
    p_i = C_i U^T + B
\end{equation}

We concatenate the outputs of the weight transformation from each parallel forward pass to a vector and apply a softmax function to this aggregate.
We compare the final representation and the ground truth label using a cross-entropy loss function $\mathcal{L}_2$ as in Eq. \ref{eq:multiple_choice_loss}.

\begin{equation}
    \label{eq:multiple_choice_loss}
    \mathcal{L}_2(p, y) = \text{CE}(\textrm{softmax}([p_1; \ldots; p_n]), y)
\end{equation}

MCGP uses the standard cross-entropy loss function because our approach treats the class imbalance problem implicitly. In MCGP, we generate examples where each polysemous word maps precisely to one choice of $k$ senses. Therefore, our method makes inference a more natural process of predicting exactly which of the $k$ senses is correct. Edge cases are words with multiple senses in one context, which we discuss further in Section \ref{sec:limitations}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% EXPERIMENTS - SETUP & DATA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% SETUP
All our models were built on top of the official BERT$_{base}$ architecture and weights, with 12 hidden layers, a hidden size of 768, a sequence length of 512, a dropout with drop probability $0.1$ on the last layer, and random shuffling during training. We initialize our prediction heads weights considering the Kaiming Uniform method \cite{HeZRS15}.
We performed the training procedures on 4 NVIDIA Tesla V100 with 16GB memory per card, an accumulated batch size of 64, the ADAM optimizer with a learning rate of $5e^{-4}$ and epsilon of $1e^{-8}$ similar to \newcite{DevlinCLT19}. The training time was, on average, 35h, 75h, and 37h, for BGP, BGP-MLM, and MCGP, respectively. The number of added parameters for BGP/BGP-M was 2\,309 as we reused the MLM head from BERT, and 18\,432 for MCGP. The maximum number of added parameters is less than 0.02\% when compared to BERT$_{base}$ (whereas KnowBERT-W+W adds over 300\% of parameters). Evaluation was performed on two GPUs (NVIDIA Tesla V100 and T4) using the official scorer from~\newcite{RaganatoCN17}\footnote{\url{http://lcl.uniroma1.it/wsdeval/}}, and considering the best results from each run. We trained on SemCor for the methods BGP and MCGP for three epochs, and BGP-M for six epochs. The complexity of learning two objectives simultaneously in BGP-M required double the training time.

% We evaluate our proposed methods in two benchmarks, namely SemCor 3.0~\cite{MillerLTB93} and GLUE~\cite{WangSMH19}. SemCor~\cite{MillerLTB93}, popular in the WSD literature~\cite{HuangSQH19,PetersNLS19}, is one of the largest manually annotated datasets with approximately 226k word sense annotations from WordNet~\cite{Miller95a}. We provide a detailed overview of this dataset in Table~\ref{table:dataset_sem}.The GLUE benchmark~\cite{WangSMH19} is a collection of nine language understanding tasks widely used in the literature~\cite{DevlinCLT19,LanCGG19} to validate transfer learning capabilities of LMs. All GLUE tasks are single sentence or sentence pair classification, except STS-B, which is a regression task. 



% Grammarly [X]
\section{Experiments} \label{sec:experiments}

In this section, we evaluate our proposed methods on two large scale benchmarks, namely SemCor 3.0~\cite{MillerLTB93} and GLUE~\cite{WangSMH19}. We first introduce the datasets, experimental setup, and details. Then, we compare \methodName~(BGP, BGP-M, and MCGP) with state-of-the-art systems. Finally, we provide the analysis and discussions of experimental results, and point out possible limitations of the presented methods.

% Grammarly [X]
\subsection{Datasets}
\label{sec:datasets}
\textbf{SemCor 3.0}~\cite{MillerLTB93}: SemCor is one of the largest manually annotated datasets with approximately 226\,000 word sense annotations from WordNet~\cite{Miller95a} for all open-class parts-of-speech. Each sentence in SemCor has multiple word annotations, and each word annotation consists of one or more sense annotations. The SemCor 3.0 corpus is commonly known and analyzed in the WSD literature~\cite{HuangSQH19,PetersNLS19}. 
We used SemCor 3.0 as training corpus for all our WSD experiments, which were validated with~\newcite{RaganatoCN17}'s framework, a set of five standardized test sets: Senseval-2~\cite{EdmondsC01}, Senseval-3~\cite{SnyderP04}, SemEval-2007~\cite{StrapparavaM07}, SemEval-2013~\cite{NavigliJV13}, and SemEval-2015~\cite{MoroN15}. We provide a detailed overview of these datasets in Table~\ref{table:dataset_sem}.

\input{tables/dataset_semeval_table}

\noindent \textbf{GLUE}: The GLUE benchmark~\cite{WangSMH19} is a collection of nine language understanding tasks widely used in the literature \cite{DevlinCLT19,LanCGG19,LiuOGD19} to validate transfer learning capabilities of language models.
All GLUE tasks are single sentence or sentence pair classification, except STS-B, which is a regression task. MNLI has three classes, and all other classification tasks have two. We use GLUE to show our models, after incorporating WSD, maintain transfer learning capabilities and increase their accuracy in natural language understanding related tasks over BERT.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% RESULTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We report the results of different transformer models peorming WSD in Table~\ref{table:model_comparison}\footnote{upon acceptance we will increase the font size}. All models are single-model singla-task and use the respective $BASE$ configuration. We observe BERT is a strong baseline and even though RoBERTa is fully converged, there was no increase in F1-score for that model. As expected, DistilBERT and AlBERT perform worse but AlBERT can keep up the performance even with 10\% BERT's parameters. From the results of BART and ELECTRA, we conclude the denoising approaches are not suitable for our WSD setup. XLNet\footnote{XLNet is the only model that makes additional use of word casing which might explain additional performance increases.} performs significantly better than BERT with almost no additional parameters which is why we choose this model compared to the BERT baseline for later experiments. All results of SemCor (Tables~\ref{table:semeval} and \ref{table:model_comparison}) report the F1 value according to the official scoring scripts~\cite{RaganatoCN17}.



We report the results of our models on the WSD evaluation benchmark~\cite{RaganatoCN17} in Table~\ref{table:semeval}. All our models are configured as single-model single-task. We evaluate the converged checkpoint of our training procedure and report the highest result for each dataset. In comparison to~\newcite{HuangSQH19}, we avoid the model bias because of frequent token insertion for transfer learning. BGP is slightly less accurate using the same number of training steps because the resulting gradients from the loss function are smaller. Incorporating the MLM objective into the training procedure also improves BGP-M results over BGP, except for SemEval2013, by a marginal difference. We assume the unexpected increase is due to the concept of discriminated fine-tuning~\cite{HowardR18}. Language models can achieve higher performance on new tasks if they optimize the MLM objective on a new corpus before fine-tuning with the task-specific objective. In our approach, we combine WSD and MLM in one pass, achieving higher accuracy on the specific task and increase its generalization.
Considering WSD as a multiple-choice problem (MCGP) increases F1-score by 4.5\% on SemEval2007 and 3.1\% on average on the \newcite{RaganatoCN17} evaluation benchmark, in comparison with GlossBERT. MCGP only performs slightly worse than the previous state-of-the-art on the SemEval2015 dataset. We assume this result is due to the relatively high number of adjectives and adverbs, and the small number of total samples in SemEval2015, which results in higher variance and sensitivity to the model. Moreover, MCGP forwards candidates for each polysemous word in parallel through the model in comparison to a sequential processing in BGP/BGP-M and GlossBERT~\cite{HuangSQH19}.

%SemEval Results
\input{tables/semeval_table}
We evaluate our suspicion that WSD training allows language models to achieve higher generalization. Hence, we fine-tune the weights from our approach in general language tasks from GLUE~\cite{WangSMH19}. Our results on the GLUE dataset show \methodName~can outperform state-of-the-art in the WSD task and successfully transfer the acquired knowledge to general language understanding datasets. The number of polysemous words in the GLUE benchmark is high in general, supporting the WSD training design of BGP-M. Appendix~\hyperref[appx:A]{A} brings more details about the polysemous words in GLUE.  We evaluated our proposed methods against previously best performing models in WSD (GlossBERT~\cite{HuangSQH19}) on the GLUE datasets. We also compared GilBERT training methods to the official BERT$_{base}$ model, achieving a 2.9\% increase in performance on average. In this work, we did not compare GilBERT to the other WSD methods performing worse than \newcite{HuangSQH19} in the WSD task (Table~\ref{table:semeval}) because reconstructing their models would have been more expensive than our entire setup, which takes up to 75h for one experiment (i.e., KnowBERT-W+W is 32\% slower). Although BGP and GlossBERT perform well in WSD, they cannot maintain good performance on other GLUE tasks. Still, BGP performs better than GlossBERT because of weak supervision without token insertion and a less biased loss function to negative examples. BGP-M outperforms BERT on most tasks and is certainly comparable to the others. Therefore incorporating MLM adds value from WSD into natural language understanding.


In comparison to other approaches, we can see a major increase over the na\"ive classification of sentence gloss pairs with BERT. Even KnowBERT W+W performs worse at task with 32\% more parameters. We show by using the best suited transformer and small adjustments in the training procedure, we can outperform GlossBERT in any task. We assume the increase of this \maskmethod over \baselinemethod is due to the concept of discriminated fine-tuning~\cite{HowardR18}. We combine WSD and MLM in one pass, achieving higher accuracy on the specific task and increase its generalization. Further, we evaluated, whether the BASE configuration of BERT is sufficient to learn representations needed for WSD. Table \ref{table:base_large} shows that the LARGE representation is not significantly better and experimental results showed that it is more prone to overfitting.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%LIMITATIONS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Grammarly [X]
\subsection{Limitations} \label{sec:limitations}
BGP-M optimizes two objectives simultaneously, so its training is more expensive than BGP and MCGP. The forward and backward passes of two different input sequences have to be temporarily stored, which reduces batch sizes by approximately 50\%. However, BGP-M adds almost no additional parameters to BERT, resulting in approximately the same inference time.

Because all proposed methods rely on a classification of one out of $k$ candidate glosses, the correct prediction of multiple senses is difficult without knowing the number of actual senses. As none of the compared approaches provide multi-sense information, and there are rare occurrences of multi-label instances (see Table \ref{table:dataset_sem}), we value this as a rather small concern in practice.

In this study, we did not include larger models (e.g., BERT$_{large}$) to maintain comparability with other methods relying on the BERT$_{base}$ architecture. However, preliminary experiments show we can outperform BERT$_{large}$ with a smaller base model by 0.4\% on average in general language understanding tasks. We leave the investigation of \methodName~with large models (e.g., RoBERTa~\cite{LiuOGD19}, ELECTRA~\cite{ClarkLLM20}) to future work as they require specialized hardware.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CONCLUSION AND FUTURE WORK
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Conclusions and Future Work}
In this paper, we presented \methodName, a set of methods (\baselinemethod, \maskmethod) to perform WSD combining BERT with lexical resources from WordNet. We proposed a method that allows for pre-training WSD, which is essential for many NLP tasks (e.g., semantic similarity). We showed our representations outperformed state-of-the-art WSD methods (+0.9\%) and improved the performance over BERT in general language understanding tasks (+2.9\%).
Even though supervised techniques require large datasets, we showed a small pre-trained model with few additional gradient steps can still make use of external knowledge of annotated corpora to improve the model. Future work will involve testing the robustness of our models on WiC~\cite{PilehvarC19}, and SuperGLUE~\cite{WangPNS19} datasets. In addition, we want to optimize the MLM objective on a new corpus before fine-tuning\cite{HowardR18}. We also plan to perform ablation studies to investigate which components of our models lead to the most benefits.

\subsection{Limitations} \label{sec:limitations}
%Because all proposed methods rely on a classification of one out of $k$ candidate glosses, the correct prediction of multiple senses is difficult without knowing the number of actual senses. As none of the compared approaches provide multi-sense information, and there are rare occurrences of multi-label instances (see Table \ref{table:dataset_sem}), we value this as a rather small concern in practice.

The obvious supervised methods is that they require sufficient labeled examples. Especially for LMGC-M this might be seen as a concern because pre-training requires large amounts of data. However, we showed that with a pre-trained model and a relatively small amount of additional gradient steps we can still use the knowledge of annotated corpora to improve the model such that a pre-training is not necessary to apply this method.

In this study, we did not include larger models (e.g., BERT$_{large}$) to maintain comparability with other methods relying on the base architecture. However, preliminary experiments show we can outperform BERT$_{large}$ with a smaller base model by 0.4\% on average in general language understanding tasks.


%%%%%%%%%%%
% Appendix
%%%%%%%%%%%

\bigskip
\newpage

\appendix

\noindent  \textbf{Appendix A. GLUE details}%\footnote{We include the Appendix in this paper and as a separate file.} \label{appx:A}

\noindent
As our experiments in Section~\ref{sec:experiments} show, the additional learning of WSD in parallel to MLM leverages our model's performance to other natural language understanding tasks. One direct result of incorporating \methodName~training methods is the increased results on the GLUE tasks. To investigate the correlation between the number of polysemous words and \methodName, we report how many words from each GLUE tasks can be found as polysemous in WordNet, as Table \ref{table:glue_polysemy} shows.

\input{tables/dataset_glue_table}

Our first observation is that the number of polysemous words in the text from different tasks is high in general. We find specific tasks like QQP with 42.8\% polysemous words in the test set with a high accuracy boost in BGP-M, but other tasks like SST-2 with 54.1\% in the test set with almost no improvement. This result indicates that although our model can understand ambiguous words, it does not necessarily mean that BGP-M will improve performance with an increased number of polysemous words. Indications for this are that the baseline model BERT$_{base}$ already has to learn WSD to some extent to perform on the GLUE datasets, and the difficulty from some tasks is not bounded to understanding polysemy. However, as our experimental results showed, on average, the performance of BGP-M is higher than the original BERT$_{base}$ model, which shows that WSD plays a role in general language understanding.
